Microwave-Assisted Tunneling in Hard-Wall InAs/InP Nanowire Quantum Dots

With downscaling of electronic circuits, components based on semiconductor quantum dots are assuming increasing relevance for future technologies. Their response under external stimuli intrinsically depend on their quantum properties. Here we investigate single-electron tunneling in hard-wall InAs/InP nanowires in the presence of an off-resonant microwave drive. Our heterostructured nanowires include InAs quantum dots (QDs) and exhibit different tunnel-current regimes. In particular, for source-drain bias up to few mV Coulomb diamonds spread with increasing contrast as a function of microwave power and present multiple current polarity reversals. This behavior can be modelled in terms of voltage fluctuations induced by the microwave field and presents features that depend on the interplay of the discrete energy levels that contribute to the tunneling process.

==> manuscript_arxiv <==
\BOOKMARK [1][-]{figure.caption.10}{References}{}% 1


==> resubmitted 2 arxiv/manuscript_arxiv <==
\BOOKMARK [1][-]{figure.caption.10}{References}{}% 1

